Wukong: Towards a Scaling Law for Large-Scale Recommendation

Scaling laws play an instrumental role in the sustainable improvement in model quality. Unfortunately, recommendation models to date do not exhibit such laws similar to those observed in the domain of large language models, due to the inefficiencies of their upscaling mechanisms. This limitation poses significant challenges in adapting these models to increasingly more complex real-world datasets. In this paper, we propose an effective network architecture based purely on stacked factorization machines, and a synergistic upscaling strategy, collectively dubbed Wukong, to establish a scaling law in the domain of recommendation. Wukong's unique design makes it possible to capture diverse, any-order of interactions simply through taller and wider layers. We conducted extensive evaluations on six public datasets, and our results demonstrate that Wukong consistently outperforms state-of-the-art models quality-wise. Further, we assessed Wukong's scalability on an internal, large-scale dataset. The results show that Wukong retains its superiority in quality over state-of-the-art models, while holding the scaling law across two orders of magnitude in model complexity, extending beyond 100 GFLOP/example, where prior arts fall short.

==> Tables/cmf.tex <==
\begin{table*}[]
\centering
\footnotesize\fontfamily{\robotofamily}\selectfont
\setlength{\tabcolsep}{1.0666em}
\begin{tabular}{lrrr}
\toprule
     & \textbf{NE}     & \textbf{Complexity}  & \textbf{QPS}        \\
     & (\%)  &  (GFLOP)   &    (P90)   \\
\midrule

\addlinespace[2px]
\multicolumn{4}{l}{\textit{Baselines}} \\
\addlinespace[2px]


DLRM, 2l & 0.38 & 1.37 & 531k \\
DLRM, 4l & 0.26 & 1.37 & 534k \\
DLRM, 4l-4x & 0.13 & 3.85 & 508k \\
DLRM, 8l-4x & 0.11 & 3.95 & 506k \\
DLRM, 4l-8x & 0.07 & 7.29 & 452k \\
DLRM, 4l-16x & 0.04 & 14.61 & 363k \\
DCN v2, 2l, r512 & +0.09 & 3.00 & 980k \\
DCN v2, 2l, r2048 & +0.07, NEX & 7.25 & 837k \\
DCN v2, 4l, r512 & +0.07, NEX & 4.42 & 912k \\
DCN v2, 8l, r512 & +0.05, NEX & 7.25 & 787k \\
FinalMLP, 4l4k-2l1k & 0.92 & 8.16 & 783k \\
FinalMLP, 4l4k-2l1k, nofs & 1.00 & 3.92 & 987k \\

\addlinespace[2px]
\hdashline
\addlinespace[4px]

\multicolumn{4}{l}{\textit{Ours}} \\
\addlinespace[2px]

Wukong, 2l & baseline & 0.53 & 963k \\
% Wukong, 2l, DC & 0.06 & & 999k \\
% Wukong, 2l, Dot & 0.03 & & 672k \\
Wukong, 4l & \textbf{-0.10} & 1.25 & 950k \\
% Wukong, 4l, DC & -0.03 &  & 941k \\
% Wukong, 4l, Dot & -0.03 & & 602k \\
Wukong, 8l & \textbf{-0.16} & 2.12 & 758k \\
Wukong, 100x & \textbf{-0.26} & 6 & 698k \\
Wukong, 300x & \textbf{-0.32} & 22.23 & 405k \\
Wukong, 500x & \textbf{-0.32} & 32.16 & 316k \\
Wukong, 1800x & & 108.04 & \\

\bottomrule
\end{tabular}
\caption{
Internal dataset, DCN frequent NEX, couldn't finish training job.
Gparams not accurate.
}
\label{tab:eval-cmf}
\end{table*}

==> Tables/criteo.tex <==
\begin{table}[h]
\footnotesize\fontfamily{\robotofamily}\selectfont
\setlength{\tabcolsep}{.9666em}
\begin{tabular}{lrr}
\toprule
                         & \textbf{AUC}     & \textbf{Complexity}        \\
                         & mean, max (std)  &  (GFLOP)          \\
\midrule

\addlinespace[2px]
\multicolumn{3}{l}{\textit{Baselines}} \\
\addlinespace[2px]

% DLRM, Slr=0.1-wmp0.1-st0.1 & 0.8058, 0.8074 (0.0013)  \\
% DLRM, Slr=0.1-wmp0.1-st0.1, d=40 & 0.8048, 0.8059 (0.0009) \\
% DCNv2, Slr=0.1-wmp0.1-st0.1        & 0.8055, 0.8072 (0.0017)                \\
% DCNv2, Slr=0.1-wmp0.1-st0.1, d=40 & 0.8051, 0.8064 (0.0013) \\
% GDCN                         & ?                \\
% FinalMLP, no FS, Slr=0.1-wmp0.1-st0.1 & 0.8055, 0.8062 (0.0005) \\
% FinalMLP, FS, Slr=0.1-wmp0.1-st0.1 & 0.8051, 0.8056 (0.0004) \\
% FinalMLP, FS-ctx, Slr=0.1-wmp0.1-st0.1 & 0.8063, 0.8068 (0.0003) \\
% Transformer                         & ?                \\

DLRM & 0.8071, 0.8074 (0.0003) & 0.0046 \\
DCNv2 & 0.8077, 0.8081 (0.0003) & 0.2623 \\
AutoInt+ & 0.8059, 0.8069 (0.0006) & \\
AFN & & \\
% MaskNet & 0.8088, 0.8101 (0.0007) & 0.0000 \\
MaskNet & 0.8082, 0.8098 (0.0010) & 0.0000 \\
FinalMLP & 0.8071, 0.8074 (0.0002) & 0.0832 \\

\addlinespace[2px]
\hdashline
\addlinespace[4px]

\multicolumn{2}{l}{\textit{Ours}} \\
\addlinespace[2px]

% DHEN, 3lc2, liang          & \fixme{0.8076, 0.8092 (0.0016)} \\
% DHEN, 3lc2, Slr=0.1 & 0.8052, 0.8064 (0.0008) \\
% DHEN, 3lc2, Slr=0.1-wmp0.5-st0.5 & {0.8078, 0.8085 (0.0005)} \\
% DHEN, 3lc2, Slr=0.1-wmp0.1-st0.1 & {0.8073, 0.8083 (0.0012)} \\
% DHEN, 3lc2, Slr=0.1-wmp0.1-st0.1, d=40 & 0.8060, 0.8069 (0.0007) \\
% DHEN, 3lc2, DSlr=0.1-wmp0.1-st0.1 & \textbf{0.8085, 0.8095 (0.0006)} \\
% Wukong, 3l & \fixme{0.8066, 0.8085 (0.0015)} \\

Wukong & \textbf{0.8086, 0.8089 (0.0002)} & 0.1702 \\

\bottomrule
\end{tabular}
\caption{Criteo grid search results over 5 repeats, Used full day 24 as test set.
}
\label{tab:eval-criteo}
\end{table}

==> Tables/dc.tex <==
\begin{table}[h]
\centering
\footnotesize\fontfamily{\robotofamily}\selectfont
\setlength{\tabcolsep}{1.0666em}
\begin{tabular}{lrrr}
\toprule
     & \textbf{NE}     & \textbf{Complexity}  & \textbf{QPS}        \\
     & (\%)  &  (GFLOP)   &    (P90)   \\
\midrule

Wukong, 2l & baseline & 0.53 & 963k \\
Wukong, 2l, DC & 0.06 & \\
Wukong, 2l, Dot & 0.03 & \\
Wukong, 4l & \textbf{-0.10} & 1.25 & 950k \\
Wukong, 4l, DC & -0.03 &  & \\
Wukong, 4l, Dot & -0.03 & & \\

\bottomrule
\end{tabular}
\caption{
Ablation study of dot compress
}
\label{tab:eval-dc}
\end{table}

==> Tables/movielens.tex <==
\begin{table}[H]
\footnotesize\fontfamily{\robotofamily}\selectfont
\setlength{\tabcolsep}{1.1666em}
\begin{tabular}{lrrr}
\toprule
 & \textbf{AUC}     & \textbf{LogLoss}  & \textbf{Complexity}     \\
                         &  &  &  (GFLOP)          \\
\midrule

\addlinespace[2px]
\multicolumn{3}{l}{\textit{Baselines}} \\
\addlinespace[2px]


DLRM & 0.9691 & 0.2150 \\ % https://openbenchmark.github.io/BARS/CTR/leaderboard/movielenslatest_x1.html
DCNv2 & 0.9691 &  0.2147 \\ % leaderboard
AutoInt+ & 0.9692 & 0.2148 \\ % leaderboard
FinalMLP & 0.9720 &  0.1966 \\ % leaderboard
% DLRM & 0.9685 & 0.2160 \\
% DCNv2 & 0.9683 &  0.2169 \\
% AutoInt+ & 0.9693 & 0.2178 \\
% FinalMLP & 0.9723 &  \textbf{0.2211} \\

\addlinespace[2px]
\hdashline
\addlinespace[4px]

\multicolumn{2}{l}{\textit{Ours}} \\
\addlinespace[2px]

Wukong & \textbf{0.9726} & 0.2488?? \\
Wukong & \textbf{0.9723} & \textbf{0.1794} \\


\bottomrule
\end{tabular}
\caption{
MovieLens results
% \fixme{TODO: run d=10 for baselines, in case they have better results.}
% \fixme{TODO: double check leaderboard}
% \fixme{add complexity?}
}
\label{tab:eval-movielens}
\end{table}

==> Tables/taobaoads.tex <==
\begin{table}[H]
\footnotesize\fontfamily{\robotofamily}\selectfont
\setlength{\tabcolsep}{1.1666em}
\begin{tabular}{lrrr}
\toprule
                         & \textbf{AUC}     & \textbf{LogLoss}     & \textbf{Complexity}    \\
                         &   & &  (GFLOP)          \\
\midrule

\addlinespace[2px]
\multicolumn{3}{l}{\textit{Baselines}} \\
\addlinespace[2px]

DLRM & 0.6386 & 0.1934 \\
DCNv2 & 0.6495  & \textbf{0.1929} \\
AutoInt+ & 0.6486 & 0.1930 \\
FinalMLP & 0.6377  & 0.1934 \\

\addlinespace[2px]
\hdashline
\addlinespace[4px]

\multicolumn{2}{l}{\textit{Ours}} \\
\addlinespace[2px]

Wukong & \textbf{0.6503} & 0.1948 \\ % d=128

\bottomrule
\end{tabular}
\caption{
TaobaoAds results
\fixme{
TODO: run d=32 for FinalMLP \& DLR, in case they have better results.
Results of Wukong, AutoInt+ and DCNv2 are final.
}
\fixme{add complexity?}
\fixme{why FinalMLP is so bad?}
}
\label{tab:eval-movielens}
\end{table}
